Fairness in the Eyes of the Data: Certifying Machine-Learning Models

We present a framework that allows to certify the fairness degree of a model based on an interactive and privacy-preserving test. The framework verifies any trained model, regardless of its training process and architecture. Thus, it allows us to evaluate any deep learning model on multiple fairness definitions empirically. We tackle two scenarios, where either the test data is privately available only to the tester or is publicly known in advance, even to the model creator. We investigate the soundness of the proposed approach using theoretical analysis and present statistical guarantees for the interactive test. Finally, we provide a cryptographic technique to automate fairness testing and certified inference with only black-box access to the model at hand while hiding the participants' sensitive data.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> sections/broader_impact.tex <==
\section*{Ethical Statement}
Our framework touches two important and sensitive subjects: fairness and privacy. As such, it has tremendous value from an ethical perspective, but also should be treated with careful consideration as a formal notion of fairness does not always align with what we think is fair and just. We believe our work is a step in the larger context of looking at Machine Learning problems through a cryptographic lens. This opens up the prospect of benefiting from what cryptography has to offer -- balancing integrity with privacy. We believe creating regulatory entities, such as our abstract entity $\Regulator$, can be a step towards standardizing fairness. Once these roles are set in place, our framework can guarantee users are treated fairly in a secure manner. 

The benefit of our framework is that it is a method to certify and evaluate fairness under a formal definition thereof, while it also conserves the privacy of clients and the intellectual property of model providers. Clients and providers benefit from it as it bridges the potential mistrust between them. It can also standardize fairness in the form of trusted regulators which are acknowledged as trustworthy in evaluating models. We find this to be an aspect that hopefully has a positive impact on society. However, we need to be careful by what we consider as fair. There is no ``one size fits all" fairness definition which complicates the validity of a certification in social terms. In particular, we focused on specific notions of fairness in our work, as these lead to an implementable result. The question of which fairness notion is the most applicable in a certain setting is independent of it and beyond the scope of this work.
Our work leaves the definition of fairness to policy makers, regulators and other experts, and gives a way to take an accepted definition of fairness and certify a model for it. It should also be noted though that we guarantee fairness only up to certain probability, and this might give people a false sense of fairness of a model even when there's a chance it is not.

%As we have shown some definitions requires less resources for statistical guarantee, it might tempt regulators to favour those definitions when they inappropriate.

What is interesting about our work is that issues like fairness and transparency are considered to be at odds with another desirable feature -- privacy. But our work brings these together. Moreover, cryptographic models for various primitives and protocols ranging from encryption to secure computation are designed to work in worst-case adversarial environments. This seems to be necessary for successful deployment of machine learning in certain applications and we hope that bringing this mindset to the machine learning field might be beneficial. 


%We also want to mention though that secure computation is not fail-proof and that e.g. the hiding of a model is only up to the resistance of the overall system to model extraction attacks.

==> sections/fairness_adjustments.tex <==
% \section{On Different Fairness Notions}\label{sec:fairness_adjustments}
% The group-based fairness definition which we used throughout the analysis in Section \ref{sec:fairness} is usually called \emph{disparate mistreatment}. This notion has multiple drawbacks: For one, it disregards the importance of each label in classification. As an example, suppose the classification task is determining if an individual would likely commit another crime~\cite{compas2016}. One might suggest that a false positive decision is much more problematic than false negative. Definition \ref{def:epsilon_fair} omits these considerations, while other definitions such as \emph{equalized odds}~\cite{hardt2016equality} do. Another example is that it does not consider a possibly biased ground-truth, when the  rate of each label should be roughly the same with respect to each group but independent of $\groundtruth$. For this we  cannot rely on measurements of group risk, but rather definitions of independence and likelihood. This fairness notion is also called \emph{demographic parity}~\cite{fairnessbook}.

% We now present necessary adjustments to the definitions and Theorem \ref{thm:sampling} for these two settings. While this does not cover all fairness notions, it gives evidence that our approach from Section \ref{sec:fairness} can be applied to some other interesting cases.

% \subsection{Equalized Odds}
% Equalized odds conditions the gap in risk between not only groups, but also labels~\cite{hardt2016equality}. We therefore need to alter the group risk (Definition \ref{def:group_risk}) as follows:  
% \begin{defn}[Group risk on $(g, y, \D)$]\label{def:eq_odds_group_risk}
% 	We define the risk of a model $M$ on group $g \in \G$ and label $y \in \Y$ as
% 	\begin{multline*}
% 	\loss{M}{g,y} = \E_{\sampsim{(x,g')}{\D}} \Big[ \indicator\left\{\classify(M,x) \neq \groundtruth(x)\right\} | \\
% 	~~~~g'=g, \groundtruth(x) = y\Big]
% 	\end{multline*}
% \end{defn}
% Accordingly, the empirical risk on sample set  $\samp{T=\{(x_1,g_1),\dots,(x_m,g_m)\}}{\D}$ would be:
% \begin{equation*}
% \emploss{M,T}{g,y} = 
% \frac{1}{m_{g,y}}\sum_{i=1}^{m} \indicator\{\classify(M,x_i) \neq y \wedge g_i=g \}
% \end{equation*}
% where $m_{g,y}$ is the number of samples in $T$ from group $g$ with label $y$.

% Following this, the definition of $\epsilon$-fair model is straightforward as the gap between groups and labels from Definition $\ref{def:eq_odds_group_risk}$. In the same way as Theorem \ref{thm:sampling} we can obtain the following
% \begin{cor}\label{cor:eq_odds_sampling}
% A model $M$ is $\epsilon$-fair with confidence $1-\delta$ if there exists a constant $ c \in (0, 1)$ such that both conditions hold
%     \begin{align*}
%         \max_{\substack{g_0,g_1 \in \G \\ y_0,y_1 \in \Y }} & \left|\emploss{M,T}{g_0, y_0} - \emploss{M,T}{g_1, y_1}\right| \leq c\epsilon\\
%         \min_{g \in \G, y \in \Y} \; \;  & m_{g,y} \geq \frac{2}{(1-c)^2\epsilon^2}\ln{\frac{2|\G||\Y|}{\delta}}
%     \end{align*}
% for $\samp{T=\{(x_1,g_1),\dots,(x_m,g_m)\}}{\D}$.
% \end{cor}
% Corollary \ref{cor:eq_odds_sampling} suggests that a larger samples set must be used in comparison to Theorem \ref{thm:sampling}. We require a minimum number of samples per group and label, instead of just per group.
% \subsection{Demographic Parity}
% Demographic parity enforces that the predicted label has the same probability across all groups~\cite{fairnessbook}. A realistic example would be a company which hires new interns and would like the acceptance rate of female and male to be roughly the same. This is a very different setting as it disregards the error the model makes completely and only cares about the tendency to predict a label per group. As such, consider the notion of likelihood with respect to a group and label: 
% \begin{defn}[Group likelihood $(g, y, \D)$]\label{def:group_likelihood}
% 	We define the likelihood of a model $M$ on group $g \in \G$ and label $y \in \Y$ as
% 	\[
% 	\likelihood{M}{g,y} = \E_{\sampsim{(x,g')}{\D}} \Big[ \indicator\left\{\classify(M,x) = y\right\} | g' = g \Big]
% 	\]
% \end{defn}
% While likelihood is usually expressed as the probability to classify the given label, since $\indicator$ is an indicator, the expectation is equal to that probability.

% The empirical group likelihood on sample set $\samp{T=\{(x_1,g_1),\dots,(x_m,g_m)\}}{\D}$ would then be
% $$\emplikelihood{M,T}{g,y} = \frac{1}{m_{g}}\sum_{i=1}^{m} \indicator\{\classify(M,x_i) = y \wedge g_i=g \}$$
% where $m_{g}$ is the number of samples in $T$ from group $g$.
 
% Adjustments for Theorem \ref{thm:sampling} are similar to the ones in Equalized Odds (Corollary \ref{cor:eq_odds_sampling}), with a key difference on measuring likelihood and $m_{g}$ instead of risk and $m_{g,y}$ (since the definition relies only on the label $y$, not $\groundtruth(x_i)$).
 
